QuantTM: Business-Centric Threat Quantification for Risk Management and Cyber Resilience

Threat modeling has emerged as a key process for understanding relevant threats within businesses. However, understanding the importance of threat events is rarely driven by the business incorporating the system. Furthermore, prioritization of threat events often occurs based on abstract and qualitative scoring. While such scores enable prioritization, they do not allow the results to be easily interpreted by decision-makers. This can hinder downstream activities, such as discussing security investments and a security control's economic applicability. This article introduces QuantTM, an approach that incorporates views from operational and strategic business representatives to collect threat information during the threat modeling process to measure potential financial loss incurred by a specific threat event. It empowers the analysis of threats' impacts and the applicability of security controls, thus supporting the threat analysis and prioritization from an economic perspective. QuantTM comprises an overarching process for data collection and aggregation and a method for business impact analysis. The performance and feasibility of the QuantTM approach are demonstrated in a real-world case study conducted in a Swiss SME to analyze the impacts of threats and economic benefits of security controls. Secondly, it is shown that employing business impact analysis is feasible and that the supporting prototype exhibits great usability.

==> chapters/2.1-RW-Table-old.tex <==
\begin{table*}[h]
\centering
\caption{Popular Threat Management Tools and Methods}
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Work}                     & \textbf{Approach} & \textbf{Importance Metric} & \textbf{Scope} & \textbf{Type} \\ \hline
\textit{Security Cards}\cite{tmmethods}& None    & None                   & Generic & Tool \\ \hline
%\textit{x}\cite{}& x    & x                   & x & x \\ \hline
\textit{OWASP TD}\cite{coretm}         & Severity Estimation & Categories (Ordinal)        & Generic & Tool \\ \hline
\textit{CAIRIS}\cite{coretm}           & Risk-based & Categories (Ordinal)        & Generic & Tool \\ \hline
\textit{TRIKE}\cite{coretm}            & Exposure Estimation & Score (Interval)       & Generic & Excel-based Tool \\ \hline
\textit{MTMT}\cite{mtmt}               & Priority Estimation & Label (Ordinal)       & Generic & Tool \\ \hline
\textit{ThreatModeler}\cite{threatm}   & Severity Estimation & Label (Ordinal)       & Generic & Tool \\ \hline
%\textit{SeaMonster}                    & ? & ? & ? \\ \hline
\textit{IriusRisk}\cite{coretm}        & Awaiting company's response & Categories (Ordinal)        & Generic & Tool \\ \hline
\textit{SDElements, securiCAD, Tutamantic}                    & \multicolumn{4}{c}{Awaiting company's response} \\ \hline
%\textit{securiCAD}                     & \multicolumn{4}{c}{Awaiting company's response} \\ \hline
%\textit{Tutamantic}                    & \multicolumn{6}{c}{Awaiting company's response} \\ \hline
\textit{Threagile}\cite{coretm}        & Risk-based & Labels (Ordinal) & Software-Integrated & Tool \\ \hline
\textit{ThreatSpec}\cite{coretm}       & None & Manual Labels & Software-Integrated & Tool \\ \hline
\textit{STRIDE}\cite{stride}           & None                & None                   & Generic & Methodology \\ \hline
\textit{LINDDUN}\cite{linddun}         & None                & None                   & Privacy & Methodology \\ \hline
\textit{DREAD}\cite{dread}             & DREAD               & Score (Interval)       & Generic & Method \\ \hline
\textit{CVSS}\cite{tmmethods}          & CVSS                & Score (Interval)       & Generic & Method and Enumeration \\ \hline
\textit{PASTA}\cite{pasta}             & PASTA               & Score (Ordinal)        & Risk-based & Method \\ \hline
\textit{PbD}\cite{jesus}               & DREAD-based         & Score (Ratio)          & Privacy & ?  \\ \hline
\cite{attackcentric}                   & Custom              & Score (Ratio)          & CPS, Software-centric & Method\\ \hline
This work                              & Economics-based     & Financial Loss (Ratio) & Generic & Method and Tool\\ \hline
\end{tabular}
\label{tab:toolsandmethodstable}
\end{table*}

